Multi-Agent Path Integral Control for Interaction-Aware Motion Planning in Urban Canals

Autonomous vehicles that operate in urban environments shall comply with existing rules and reason about the interactions with other decision-making agents. In this paper, we introduce a decentralized and communication-free interaction-aware motion planner and apply it to Autonomous Surface Vessels (ASVs) in urban canals. We build upon a sampling-based method, namely Model Predictive Path Integral control (MPPI), and employ it to, in each time instance, compute both a collision-free trajectory for the vehicle and a prediction of other agents' trajectories, thus modeling interactions. To improve the method's efficiency in multi-agent scenarios, we introduce a two-stage sample evaluation strategy and define an appropriate cost function to achieve rule compliance. We evaluate this decentralized approach in simulations with multiple vessels in real scenarios extracted from Amsterdam's canals, showing superior performance than a state-of-the-art trajectory optimization framework and robustness when encountering different types of agents.

==> tex/notes.tex <==
\clearpage

\mycyan{\section{Notes}}

Remarks after review (8.8.22):

\textbf{Intro:}
\begin{itemize}
    \item Shorten
    \item Contribution as subsection (e. g. rule-based cost, 2 stage evaluation, ...)
    \item Make more clear that we are able to plan and predict in one step
    \item May point out that we could introduce "rational behaviour" with the hand-shaped cost function. (as its written now, one could get the impression that it only works if everything is nice, smooth and rational.)
    \item 
\end{itemize}

\textbf{Related work:}
\begin{itemize}
    \item May add the references from the review (or others?)
    \item Currently we say a lot why other stuff doesn't work, may we reduce that and just say what they did? Then summarize what the current state is and why ours is better without saying others are bad?
    \item It's also very extensively explained what is done and how, may reduce?
    \item 
\end{itemize}
\textbf{Preliminaries:}
\begin{itemize}
    \item Global planning: Make more clear that the local goal gives more of a "general direction of travel"
    \item 
\end{itemize}

\textbf{Approach:}
\begin{itemize}
    \item ok to me in general
    \item may swap from $k_{min}$ cut to copying individual samples up to  $k_max$?
    \item Drop explanation why we drop the variance cost term (variance from warmstart)
\end{itemize}

\textbf{Experiments:}
\begin{itemize}
    \item At first glance (and after 3 months ignoring it) i understand why one could get the impression that we tested only with the two maps shown.
    \item Drop Fig 7: Fig 6 and 7 could be combined e.g. show the "avoid to right" and "decelerate" maneuvers in a 4 agent plot: Replace Fig 6l with 7, 6m with Prinsengracht plot?
    \item What do we want to do with 6l? On one side its needed to prove that it works with the autonomous setup (wrt to the "failing" mode with aggressive vessels) on the other side it does not say that much imo.
    \item Update and append the table with 4 agent experiments. Drop arrival times
    \item LMPCC comparison, how do we want to set it up?
    \item Introduce randomization (do not run the same experiment over and over again: implemented in feature/randomizedStatsGen
    \item What about the thight crossing? On one side it proves that it works in very tight spaces, on the other hand people might say that its to "simple" e.g. too far off a real canal
    \item Make more clear that cooperative human drivers create identical trajectories compared to the fully autonomous setup
    \item May adapt section on computational complexity. Fig 9 uses a lot of space for not showing that much.
    \item 
\end{itemize}

\textbf{Conclusion:}
\begin{itemize}
    \item Adapt according to what we state in the contribution. e.g. Stress more on the simultaneous predict and plan
    \item State that it actually runs real-time w. up to 4 agents on a CPU, GPU req. for more vessels eventually
    \item GPU implementation and cost/intention/goal estimation on as outlook
\end{itemize}

\textbf{final adjustments}
\begin{itemize}
    \item Make plots the same (ruler instead of axis) and colorblind friendly
    \item fix image quality
    \item four agents maybe get rid of label or start from agent 1 not 0
    \item references
    \item Correct rule violation figure
    \item Check that we are actually talking enough on how are method compares to the state of the art
\end{itemize}


\begin{comment}


\mycyan{\section{Notes}}

\textbf{Task list:}

Preliminaries:
\begin{itemize}
    \item Shorten MPPI theory
    \item Might put shortened algorithm?
\end{itemize}

Approach:
\begin{itemize}
    \item Clarify formulation
    \item Replace optimization plot (gray background)
\end{itemize}

Experiments
\begin{itemize}
    \item Complete computation times part
\end{itemize}

Others:
\begin{itemize}
    \item Write Abstract, Summary
    \item Check that bibliography is complete, correct and consistent. Change arxiv papers to peer reviewed version
\end{itemize}


\textbf{Schedule}
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
 Date & Section TODO  \\
  \hline\hline
     Tu 8. &  \\ 
     We 9. & Related Work \\ 
     Do 10. &  \\ 
     Fr 11. & Approach \\ 
     Sa 12. &  \\ 
     So 13. & Experiments \\ 
     Mo 14. &  \\ 
     Tu 15. & Abstract, Summary, Outlook \\ 
     We 16. & READY for review \\ 
 \hline
\end{tabular}
\end{center}

The current \mycyan{plan} for completing the paper is the following:
\mycyan{\begin{enumerate}
\item Related work: 
\end{enumerate}}

\textbf{Selling-points/Contribution}
\begin{itemize}
    \item Decentralized interaction-aware motion prediction and control for multiple vessels/agents
    \begin{itemize}
        \item Faster, no simplifications
        \item Distributed and no communication
        \item Control and Predict at the same time (Interaction awareness)
        \item Simple local goal prediction with constant velocity assumption
    \end{itemize}
    \item 
\end{itemize}


\textbf{Approach on writing}
\begin{itemize}
    \item Local planning with MPPI for vessels
    \item (higher level)
\end{itemize}

\textbf{Things to change/improve}
\begin{itemize}
    \item Fix statistics for collisions -> a bit more margin for collisions
    \item Improve representation
    \item 
\end{itemize}


%%%%%%%%
\textbf{Thoughts collection for related work:}
%%%%%%%%

\subsection{Navigation among crowds}
The navigation in crowds is major challenge for mobile robotic systems.

Classic reaction based, seen at least 5 times in papers)
\begin{itemize}
    \item RVO (Van den Berg, 2008), ORCA (van den Berg, 2011): one step interaction for geometric configuration.
    \item No consideration of evolution of neighboring agents which can lead to oscillatory and undesired behaviour.
    \item DWA (fox) for considering dynamic obstacles with constant velocities.
    \item 
\end{itemize}
Problem of predict-plan structure: The action of other agents is dependant on ours and vice-versa. So the motion assumption is too general, not interaction-aware, in tight (canal) environments or crowded scenarios. \\
\\
Communication-capable and or centralized systems:
\begin{itemize}
    \item Looking for joint optimal solutions by communicating state and goals, trajectories
    \item Reducing state space by looking into pair wise configurations
    \item See refs of Brito "Where to go next" and Chen 2017 "Decentralized non-communicating multi agent collisions"
    \item \textbf{find some refs for these!}
\end{itemize}
Issues are computation times and the missing capabilities of to deploy centralized or communicating methods in canal environment with human driver. 

Learning based:
\begin{itemize}
    \item Brito: Where to go next (Subgoals, motion crowds, with MPC)
    \item Chen: Decentralized Non-comm (Learned avoiding behaviour with encoded/integrated goal estimation)
    \item Chen: Socially-aware Motion-planning (introducing right-handed rules)
    \item Kuderer: feature based trajectory predictions
    \item Kretzschmar: Social Compliant mobile robot navigation (IRL)
    \item Park: Social Trajectory planning for ASVs with KDE  (Data-drive, IRL)
\end{itemize}
The major limitation for learning based approaches is the issue of generalization. The underlying model is not accessible therefore the outcome of a run is not predictable.


\subsection{Autonomous Driving}
In the autonomous driving sector can be 
Similar techniques than navigation among crowds, more reinforcement learning and game theory.
(Classification retrieved from Brito, Learning Interaction-aware guidance)

Rule based methods (in autonomous driving):  Policies
\begin{itemize}
    \item Paden: "A survey of motion planning and control techniques for self-driving urban vehicles"
    \item Mostly applied in structured environments (intersections, lane changing) works well for low volume traffic situations
    \item problems when margin becomes smaller, freezing robot problems 
\end{itemize}

Search based:
\begin{itemize}
    \item Intention-aware online POMDP (Bai)    
    \item Li: Behavior and Interaction-aware Motionplanning: RL for pattern-intention-motion models learning, POMDP for risk bounded motion plans
\end{itemize}

Learning based methods:
\begin{itemize}
    \item Brito: Learning interaction aware guidance policies (Autonomous driving, intersections)
    \item 1-2 more examples
\end{itemize}

Optimization based autonomous driving: Find examples
\begin{itemize}
    \item time-critical with accurate models and larger sets of motion primitives / system agents
    \item Explicit collision and kino-dynamic constraints definitions
    \item Simple, interaction free predictions, non-ego motion is not considered
    \item Roboat papers (non interaction aware MPC)
    \item De fries, Regulation Aware motion planning 
    \item Ji, Path Planning and Tracking for Vehicle Collision Avoidance: 3-D virtual dangerous potential field, with MPC tracking the resulting trajectory. Predict, Plan approach
\end{itemize}

Game theoretic approaches:
\begin{itemize}
    \item modelling social interactions
    \item Social Value orientation (SVO) used to classify human driving behaviour: altruistic vs egoistic (aka breaking for a left turning car or go on in unprotected left turning cycles)
    \item UKF to estimate cost params for other agents -> find paper for this!
    \item Schwarting: Social behaviour of AV (two papers) -> Estimation of SVO
    \item Le Cleac'h AL game: 3s horizon, circular collision check, probably doesn't work with tight intersections, solving for a fixed set of strategies Otherwise quite promising tbh
    \item Fridovich-Keil, ilqGames solver: Solving repeated linear-quadratic games
\end{itemize}
%%%%%%%%
%% end initial thoughts collection
%%%%%%%%
Intror text: Rel work
In the field of dynamic motion planning there are two main areas identified where this capability is key. On one hand there is the autonomous mobile robot sector where agents are supposed to navigate in crowds of pedestrians. On the other hand there is the autonomous driving field where we see methods resolve the situation of crossing an intersection or entering a highway. For both fields it is possible to distinguish between reaction-based  and truly interaction-aware planning. 


%%%% START OLD ADAPTED MPPI ALGORITHM:
\begin{algorithm}
\caption{Adapted MPPI}\label{alg:mppi_adapted_short_old}

\begin{algorithmic}
\State \textbf{Given} $\mathbf{U}_t$, $\mathbf{q}_{t_0}$: previous control sequence (hot start), current system state
\State $\mathbf{p}_t \rightarrow $ \textit{receiveEgoLocalGoal()}
\State $\mathbf{p}_{t,i} \rightarrow $\textit{predictLocalGoal()} \textit{predictLocalGoals($\mathbf{q}_{t_0}$)}
\For{$i \leftarrow 0$, $i < n$} // for every agent
    \For{$k \leftarrow 0$, $k < K$} // for every sample
        \State Sample $\mathcal{E}_i^k = (\epsilon^k_{i,0} \dots \epsilon^k_{i,T-1}), \quad \epsilon^k_t \in \mathcal{N}(0, \nu \Sigma)$
        \State $\mathbf{V}_i^k = \mathcal{E}_i^k + \mathbf{U}_i$
        \State Predict $\mathbf{Q}_i^k \leftarrow$ \textit{simSystem($\mathbf{V}_i^k, \mathbf{q}_{i, t_0}$)}
        \State  $S_i^k \leftarrow$ \textit{getIndividualCost($\mathbf{Q}_i^k$, $\mathbf{V}_i^k$)}
        \If{$S_i^k > C_{\text{collision}}$}
           \State Drop sample $ \mathcal{E}_i^k, \mathbf{Q}_i^k, S_i^k$
           \State \textbf{break}
        \EndIf
    \EndFor
\EndFor

\State Unify samples to agent with fewest;

\For{$k \leftarrow 0$, $k < K$}
    \State $\mathcal{S}^k = \sum_{i =0}^{n-1}S_i^k + $         \textit{getConfigurationCost($\mathbf{Q}^k$)}
\EndFor

\State $\mathbf{w}$ = \textit{importanceSample($\mathcal{S}$)};

\State return $\mathbf{U}_{t+1} = \mathbf{U}_t + \mathbf{w} \mathcal{E}_i^k$;


\end{algorithmic}
\end{algorithm}





\end{comment}


\begin{comment} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% First version of State and dynamics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The multi agent state is related to Williams \cite{williams_model_2017} work with Simulated Multi Rotors in a Forrest. The system state $q$ is formed by stacking the individual states 
\begin{equation}\label{eq::dynamics}
    \mathbf{q}_i = \begin{pmatrix}  \mathbf{x}_i &
                                    \mathbf{v}_i \end{pmatrix}^T
    = \begin{pmatrix} x_i &  y_i & \phi_i  & u_i & v_i & \dot{\phi}_i \end{pmatrix}^T
\end{equation}
for every agent to an entire system of agents. This is stated as 

\begin{equation} \label{eq::state}
    \mathbf{q} = \begin{pmatrix}
    \mathbf{q}_0 &
    \mathbf{q}_1 &
    \hdots &
    \mathbf{q}_{n-1} &
    \mathbf{q}_n &
    \end{pmatrix}^T.
\end{equation}
%The dynamics model is chosen as suggested in previous work on the ROBOAT platform \cite{wang_design_2018,wang_roboat_2019,wang_roboat_2020}. Therefore we model the dynamic as a nonlinear second order system. We discard Coriolis and centripetal effects since the vessel always sails at low speeds. Therefore we state 
\begin{equation}
    \begin{pmatrix} \dot{\mathbf{x}}_{i} \\
    \dot{\mathbf{v}}_{i}\end{pmatrix}
     = \begin{matrix}
    \mathbf{R}_i(\phi_i)
    \mathbf{v}_i(t) \\
    \mathbf{M}^{-1}\big(\mathbf{B}\mathbf{u}_i(t) - \mathbf{D}(\mathbf{v}_i(t)) \mathbf{v}_i(t)\big)
    \end{matrix}
    \end{equation}
    % \mathbf{M}^{-1}\bigg(\mathbf{B}\mathbf{u}_i(t) - \big(\mathbf{C}(\mathbf{v}_i(t)) + \mathbf{D}(\mathbf{v}_i(t))\big) \mathbf{v}_i(t) \bigg)
%with parameters representing $\mathbf{R(\phi_i)}$ transformation matrix from body to inertial frame, mass matrix $\mathbf{M}$, applied forces (thrust) $\mathbf{B}\mathbf{u}_i(t)$ and drag matrix $\mathbf{D}(\mathbf{v_i}(t))$ as
\begin{equation}
    \mathbf{R(\phi_i)} = \begin{pmatrix}
    \cos(\phi_i) & -\sin(\phi_i) & 0 \\
    \sin(\phi_i) & \cos(\phi_i) & 0 \\
    0 & 0 & 1 \\
    \end{pmatrix},
\end{equation}
\begin{equation}
    \mathbf{M} = \text{diag} \{m_{11}, m_{22}, m_{33} \},
\end{equation}
\begin{equation}
    \mathbf{B}\mathbf{u}_i(t) = 
        \begin{bmatrix} 1 & 1 & 0 & 0 \\
            0 & 0 & 1 & 1 \\
            \frac{a}{2} & -\frac{a}{2} & \frac{b}{2} & -\frac{b}{2} 
        \end{bmatrix}
        \begin{pmatrix}
            f_1 \\ f_2 \\ f_3 \\ f_4
        \end{pmatrix}
\end{equation}


\begin{equation}
    \mathbf{D}(\mathbf{v_i}(t)) = \text{diag} \{X_u, Y_v, N_r \}.
\end{equation}

\subsection{MPPI Theory} \label{sec:mppi_theory}
%In this section we will show an introduction to the main key concepts of the MPPI based on the information theoretic framework. For detailed derivations and insights on its connections to stochastic optimal control we refer the reader to (Williams2018).
%We will start by defining a function:
\begin{equation}
    \mathcal{F}(S, \mathbb{P}, x_0, \lambda)  = -\lambda \log \left\{\mathbb{E_P}\left[ \text{exp}\left(-\frac{1}{\lambda} S(V)\right)\right] \right\}
\end{equation}
%which we will denote as free-energy of the control system. Here, $V$ is a sequence of inputs, $S(V)$ is the state dependent cost given an input sequence, $\lambda$ is a tuning parameter defined as the system's inverse temperature, $x_0$ is the initial state of the system and $\mathbb{P}$ is a base measure, usually a probability distribution over the inputs of the uncontrolled system. It can be shown that: 
\begin{equation} \label{eq::free_energy_ineq}
    \mathcal{F}(S, \mathbb{P}, x_0, \lambda) \leq \mathbb{E_Q}[S(V)] + \lambda \mathbb{KL}(\mathbb{Q}||\mathbb{P})
\end{equation}
%where $\mathbb{Q}$ is a probability measure representing the controlled input distribution and $\mathbb{KL}(\mathbb{Q}||\mathbb{P})$ is the KL-Divergence between the base and controlled measured. The above equation means that the free-energy acts as a lower bound to an expected state dependent cost and the KL-Divergence, which acts as a control cost. We can now define a new measure $\mathbb{Q}^*$ through its Radon-Nikodym derivative with respect to the base measure:
\begin{equation}\label{eq::RN_der}
    \frac{d\mathbb{Q^*}}{d\mathbb{P}} = \frac{\exp(-\frac{1}{\lambda} S(V))}{\mathbb{E_P}[\exp(-\frac{1}{\lambda} S(V))]}
\end{equation}
%Substituting $\mathbb{Q}$ with $\mathbb{Q}^*$ in eq.\eqref{eq::free_energy_ineq} we can prove that $\mathbb{Q}^*$ is the optimal control distribution in the sense that it achieves the lower bound.
%The idea is now to align our control distribution $\mathbb{Q}$ with the optimal distribution $\mathbb{Q}^*$ though KL minimization:
\begin{equation}\label{eq::info_optimal_input}
    U^* = \argmin_U \mathbb{KL(Q^*||Q)}
\end{equation}
Considering now a discrete time system:
\begin{equation}
    x_{t+1} = F(x_t, v_t),   \quad   v_t \sim \mathcal{N}(u_t,\Sigma)
\end{equation}
%where $x_t \in \mathbb{R}^n$ is the state vector, $v_t \in \mathbb{R}^m$ is the noisy input and $u_t \in \mathbb{R}^m$ is the commanded input. If our measures $\mathbb{P}$ and $\mathbb{Q}$ are defined through their probability density functions as:
\begin{equation}
    \begin{aligned}
    & \quad p(V) = \prod_{t=0}^{T-1} \frac{1}{((2\pi)^m |\Sigma|)^{1/2}} \exp \left( -\frac{1}{2} v_t^T \Sigma^{-1} v_t \right)\\
    & q(V|U) = \\ & \prod_{t=0}^{T-1} \frac{1}{((2\pi)^m |\Sigma|)^{1/2}} \exp \left( -\frac{1}{2} (v_t-u_t)^T \Sigma^{-1} (v_t-u_t) \right)
    \end{aligned}
\end{equation}
%we can prove that the optimal control input at time $t$ is the mean input under the optimal distribution.
\begin{equation}\label{eq::Williams_optimal_in}
    u_t^* = \int_{\Omega_V} q^*(V) v_t dV,
\end{equation}
%Since we cannot sample from the optimal distribution, we cannot easily estimate the mean though Monte Carlo sampling. What we can do instead, given eq.\eqref{eq::RN_der}, is to define an importance sampling scheme that allows us to estimate the optimal control input at time $t$ by sampling around our controlled distribution:
\begin{equation}
\begin{aligned}
    &\omega(V) =\\ & \frac{1}{\eta} \exp \left( - \frac{1}{\lambda} \left( S(V) + \frac{\lambda}{2} \sum_{t=0}^{T-1} u_t^T \Sigma^{-1} u_t + 2u_t^T \Sigma^{-1} \epsilon_t \right) \right),\\
    & \quad u_t* = \mathbb{E_Q}[\omega(V)v_t]\\
\end{aligned}
\end{equation}

\end{comment}

==> tex/previous_work.tex <==
\section{Related Work} \label{sec:prevwork}
% In the following we split methods into reactive and interaction-aware planning. We consider reactive methods as approaches being aware of dynamic obstacles.

\subsection{Reactive Planning}
Most autonomous mobile robots in industry are deployed with reaction-based methods. The oldest and most well-known examples are the Dynamic Window Approach (DWA) \cite{fox_dynamic_1997}, Reciprocal Velocity Obstacle (RVO) \cite{van_den_berg_reciprocal_2008} or its extension Optimal Reciprocal Collision Avoidance (ORCA) \cite{van_den_berg_reciprocal_2011}. The ego-agent predicts the motion of all other agents (e.g. using a constant velocity assumption \cite{fox_dynamic_1997} or geometric rules \cite{van_den_berg_reciprocal_2011}) to compute a corresponding collision-free trajectory. For longer horizon plans Artificial Potential Fields (APF) are often considered. Examples are shown for avoiding humans \cite{svenstrup_trajectory_2010} or autonomous vehicles \cite{ji_path_2017} where a path is extracted via Rapidly-exploring Random Trees (RRT) or graph search, which will then be tracked by lower-level controllers such as PID, LQR or MPC.

MPC can also be utilized as a local planning framework considering obstacles explicitly. Recent work within the ROBOAT project presents regulation-aware obstacle avoidance \cite{de_fries_regulations_2021} by interpreting canal regulations as cost terms and considering other vessels as constant velocity obstacles. In free-space scenarios and low traffic configurations these approaches show great performance. For more complex scenarios with dense environments or multiple dynamic agents, MPC-based algorithms tend to fail and can lead to frozen robots \cite{trautman_unfreezing_2010} or worse, collisions.

\subsection{Interaction-aware Planning}
Considering the limitations discussed above, it is clear that better anticipation of other agents is required. However, behavior modeling and estimation is challenging for crowds of pedestrians or human piloted vehicles. Model-based estimation methods, such as social forces \cite{helbing_social_1995}, often only consider one type of agent in the crowd (such as humans) to enable scalability. Thus, they struggle to incorporate more specific behaviors that may arise, for example, due to agent-specific kinodynamic constraints.

Several learning-based methods have been proposed to address this problem. Kuderer et al.~\cite{kuderer_feature-based_2013} and Kretschmar et al.~\cite{Kretzschmar} present deep-learned trajectory predictions for humans, while Park et al.~\cite{park_social_2021} introduced a social planner for ASVs. These learned predictions can then be used to replace APF methods. Alternatively, Brito et al.~\cite{brito_where_2021} skip the explicit prediction of other agents and implicitly encode interaction-awareness in the deep-learned policy that generates local subgoals for the MPC.

% Now we consider that the presence of the ego-agent affects the plan of other agents but actions of the ego-agent are still not considered. 

Indeed, works that incorporate interaction-awareness into motion planning often consider the behavior of the entire system of agents. This has been demonstrated for Gaussian process-based~\cite{trautman_robot_2013} as well as deep learning-based~\cite{chen_decentralized_2017} modeling methods. The latter work was extended to incorporate social rules~\cite{chen_socially_2018}, while Riviere et al.~\cite{riviere_glas_2020} generalized this even further by including global path planning. In these works, the dependency of the agent actions and intentions are therefore encoded inside the deep networks.

% Such inter-agent dependency can also be treated as negotiation. Game theory approaches tackle these kinds of problems by searching for the individual optimum based on the actions of other agents. Fridovich-Keil et al.~\cite{fridovich-keil_efficient_2020} as well as Le Cleac'h et al.~\cite{le_cleach_algames_2020} propose solving for optima related to local Nash-equilibria under the assumption of accessible strategies. Schwarting et al.~\cite{schwarting_planning_2018, schwarting_social_2019} further aims to estimate each agent's strategy in the form of its Social Value Orientation (SVO) to account for more egocentric or altruistic agents. 
% Instead of of looking for each agent's optimum, we can also search for the overall system optimum (as intended in a urban traffic systems) and perform centralized planning as in \cite{wagner_m_2011} (multi-agent A*) or (Ferner, 2013), (Cirillo, 2014), (Yu, 2016). In practice, these approaches require knowledge of each agent's state and goal, and all the agents have to follow the centralized instructions, which is computationally demanding especially for complex environments.

\subsection{Model Predictive Path Integral Control}
% To address the computational load, MPPI promises an interesting alternative. It was is intended to provide approximated solutions of stochastic optimal control problems through the use of sampling \cite{kappen_path_2005}. This is desirable especially for complex non-convex optimization tasks. At first, it was then implemented in a Model Predictive Control (MPC) fashion to race a rally car at to its physical performance limit around a dirt track \cite{Williams2015, Williams2016}. In later works, a new formulation for Model Predictive Path Integral (MPPI) control based on an information theoretic framework  was derived to allow for optimizing a larger class of systems, including those that are not affine in control \cite{Williams2016a, Williams2017,Williams2018a}. 
% Thanks to the sampling based nature of MPPI we can solve non-linear, non-convex, discontinuous stochastic optimal control problems without the need for any simplification. Compared to other stochastic optimal control methods as iterative Linear Quadratic Gaussian (iLQG) \cite{li_iterative_2007} or Differential Dynamic Programming (DDP) \cite{Theodorou2010a}, MPPI does not require linearization of the dynamics of the system and quadratic approximation of the cost function, and therefore does not require differentiability and has a considerable advantage whenever the aforementioned approximations are hard to make.
% MPPI was proven to be a computationally efficient centralized method for motion planning of multiple agents \cite{williams_model_2017}. The next step is to introduce regulation awareness and investigate upon which stage the method is suitable for a decentralized, non-communicating and interaction-rich setting.

In contrast to learning-based methods, optimization strategies such as MPC and MPPI directly solve for the best control trajectory at each step by forward simulating the behavior of the full system. In particular, MPPI uses a sampling-based framework~\cite{kappen_path_2005} to rollout simulations, allowing it to solve non-linear, non-convex, discontinuous stochastic optimal control (SOC) problems~\cite{Williams2015,Williams2018a}. Compared to other SOC methods such as iterative Linear Quadratic Gaussian (iLQG) \cite{li_iterative_2007} or Differential Dynamic Programming (DDP) \cite{Theodorou2010a}, MPPI does not require linearization of the system dynamics or quadratic approximation of the cost function, and therefore does not require differentiability and has a considerable advantage whenever the aforementioned approximations are hard to make. This makes MPPI particularly well-suited to our target task of ASV navigation in urban canals since the interaction-based regulations explicitly give rise to non-differential costs. In addition, \cite{williams_model_2017} showed MPPI to be a computationally efficient centralized method for multi-agent motion planning. Thus, in this work, we introduce a method for decentralized multi-agent motion planning via MPPI in non-communicating and interaction-rich settings.

%Overview:
%\begin{itemize}
%    \item Related roboat papers and current state for vessels
%    \item Interaction aware planning, multi agent setup, Centralized, Decentralized motion planning (Game theory, RL
%    \item Williams papers and other applications of MPPI
%\end{itemize}

